Asymptotically preserving particle methods for strongly magnetizedplasmas in a torus

We propose and analyze a class of particle methods for the Vlasov equation with a strong external magnetic field in a torus configuration. In this regime, the time step can be subject to stability constraints related to the smallness of Larmor radius. To avoid this limitation, our approach is based on higher-order semi-implicit numerical schemes already validated on dissipative systems [3] and for magnetic fields pointing in a fixed direction [9, 10, 12]. It hinges on asymptotic insights gained in [11] at the continuous level. Thus, when the magnitude of the external magnetic field is large, this scheme provides a consistent approximation of the guiding-center system taking into account curvature and variation of the magnetic field. Finally, we carry out a theoretical proof of consistency and perform several numerical experiments that establish a solid validation of the method and its underlying concepts.

==> macro.tex <==
\usepackage{amsthm,amsfonts,amssymb,amsmath,oldgerm}
\numberwithin{equation}{section}
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{setspace}
\usepackage{stmaryrd}
\usepackage{mathrsfs}
\usepackage{fancyhdr}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{bm}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{multirow}
\usepackage{psfrag}
\usepackage[font=scriptsize]{caption}
\usepackage[font=scriptsize]{subcaption}
\usepackage{listings}
\usepackage{tikz}
\usepackage{empheq}
\usepackage{cases}
\usetikzlibrary{matrix} 
\usepackage[framemethod=TikZ]{mdframed}
\mdfdefinestyle{MyFrame}{backgroundcolor=gray!20!white}
\usepackage[makeroom]{cancel}

\usepackage[top=20mm,bottom=20mm,left=18mm,right=18mm,a4paper]{geometry}

% \usepackage{showkeys}
\usepackage{hyperref,bookmark}

%\usepackage[normalem]{ulem}
%\normalem
%\definecolor{violet}{rgb}{0.580,0.,0.827}
%\def\corr#1#2#3{\typeout{Warning : a correction remains in page
%\thepage}
%\textcolor{blue}{\sout{#1}}
%\textcolor{violet}{#2}
%\textcolor{red}{#3}}
%\usepackage[textwidth= \marginparwidth,textsize=tiny]{todonotes}
%\DeclareRobustCommand{\vect}[1]{\bm{#1}}
%\pdfstringdefDisableCommands{%
%  \renewcommand{\vect}[1]{#1}%
%}
\hypersetup{
    colorlinks,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=blue,      % color of file links
    urlcolor=blue,           % color of external links
    linkcolor=blue,
}
%\allowdisplaybreaks

%wider margins? (NO DIFFERENCE IN LENGTH) 
%\setlength{\evensidemargin}{0in}
%\setlength{\oddsidemargin}{0in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Makros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
\newcommand{\ols}[1]{\mskip.5\thinmuskip\overline{\mskip-.5\thinmuskip {#1} \mskip-.5\thinmuskip}\mskip.5\thinmuskip} % overline short
\renewcommand\d{\partial}
\newcommand\dD{\mathrm{d}}
\newcommand\eD{\textrm{e}}
\newcommand\iD{\textrm{i}}
\newcommand\ii{\iD}
\newcommand\dd{\dD}
\def\eps{\varepsilon }
\newcommand\errfn{\textrm{errfn}}
\newcommand{\Id}{{\rm Id}}
\newcommand{\A}{{\rm \bA}}
\newcommand{\J}{{\mathcal J}}
\newcommand{\I}{{\rm I}}
\newcommand{\Range}{{\rm Range }}
\newcommand{\Span}{{\rm Span }}
\newcommand{\Res}{{\rm Residue}}
\newcommand{\sgn}{\text{\rm sgn}}
\newcommand{\sign}{{\text{\rm sgn }}}
\newcommand{\const}{\text{\rm constant}}
\newcommand{\diag}{{\rm diag }}
\newcommand{\intl}{[\![}
\newcommand{\intr}{]\!]}
\newcommand{\mueq}{\cM_{\rho_0/\eps,\cV}\otimes\bar{\mu}_{t,\bx}}
\newcommand{\mueqeps}{\cM_{\rho_0/\eps,\cV^}\otimes\bar{\mu}_{t,\bx}}
%%%%%%%%%%%%%%%%%%

\newcommand\br{\begin{remark}}
\newcommand\er{\end{remark}}
\newcommand\bp{\begin{pmatrix}}
\newcommand\ep{\end{pmatrix}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand\ba{\begin{equation}\begin{aligned}}
\newcommand\ea{\end{aligned}\end{equation}}
\newcommand\ds{\displaystyle}
\newcommand\nn{\nonumber}
\newcommand{\beg}{\begin{example}}
\newcommand{\eeg}{\end{exaplem}}
\newcommand{\bpr}{\begin{proposition}}
\newcommand{\epr}{\end{proposition}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{corollary}}
\newcommand{\ec}{\end{corollary}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\newcommand{\brs}{\begin{remarks}}
\newcommand{\ers}{\end{remarks}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{example}[theorem]{Example}
\newtheorem{notation}[theorem]{Notational convention}

\newtheorem{obs}[theorem]{Observation}
%\numberwithin{equation}{section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\cf}{\textit{cf.} }
\newcommand{\etal}{\textit{et al.\ }}
\def\mm#1{\begin{align}#1\end{align}}
\def\mmn#1{\begin{align*}#1\end{align*}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cn}{\operatorname{cn}}
\newcommand{\one}{\bm{1}}
\newcommand{\grandO}{\cO}

%\DeclareMathOperator{\Div}{div}

\newcommand{\intg}{[\![}
\newcommand{\intd}{]\!]}

%\renewcommand{\AA}{{\mathbb A}}
\newcommand{\BB}{{\mathbb B}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\DD}{{\mathbb D}}
\newcommand{\EE }{{\mathbb E}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\II}{{\mathbb I}}
\newcommand{\JJ}{{\mathbb J}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\MM}{{\mathbb M}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\OO}{{\mathbb O}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
%\renewcommand{\SS}{{\mathbb S}}
\newcommand{\TT}{{\mathbb T}}
\newcommand{\UU}{{\mathbb U}}
\newcommand{\VV}{{\mathbb V}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\XX}{{\mathbb X}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\ZZ}{{\mathbb Z}}

\newcommand{\AM}{{\mathbb A}}
\newcommand{\BM}{{\mathbb B}}
\newcommand{\CM}{{\mathbb C}}
\newcommand{\DM}{{\mathbb D}}
\newcommand{\EM }{{\mathbb E}}
\newcommand{\FM}{{\mathbb F}}
\newcommand{\GM}{{\mathbb G}}
\newcommand{\HM}{{\mathbb H}}
\newcommand{\IM}{{\mathbb I}}
\newcommand{\JM}{{\mathbb J}}
\newcommand{\KM}{{\mathbb K}}
\newcommand{\LM}{{\mathbb L}}
%\newcommand{\MM}{{\mathbb M}}
\newcommand{\NM}{{\mathbb N}}
\newcommand{\OM}{{\mathbb O}}
\newcommand{\PM}{{\mathbb P}}
\newcommand{\QM}{{\mathbb Q}}
\newcommand{\RM}{{\mathbb R}}
\newcommand{\SM}{{\mathbb S}}
\newcommand{\TM}{{\mathbb T}}
\newcommand{\UM}{{\mathbb U}}
\newcommand{\VM}{{\mathbb V}}
\newcommand{\WM}{{\mathbb W}}
\newcommand{\XM}{{\mathbb X}}
\newcommand{\YM}{{\mathbb Y}}
\newcommand{\ZM}{{\mathbb Z}}

%%%%%%%%%%%%
\newcommand\bj{{j}}
\newcommand\bk{{\bm k}}
\newcommand\bll{{\bm l}}
\newcommand\bmm{{\bm m}}
\newcommand\bx{{\bm x}}
\newcommand{\bz}{\bm z}
\newcommand{\by}{\bm y}
\newcommand{\bh}{\bm h}
\newcommand{\bxi}{\bm \xi}
\newcommand{\bdel}{\bm \delta}
\newcommand{\ber}{\bm e}
\newcommand{\bu}{\bm u}
\newcommand\bv{{\bm v}}
\newcommand\Div{{\rm div}}



%%%%%%%%%%%%
\newcommand\bA{{\mathbf A}}
\newcommand\bB{{\mathbf B}}
\newcommand\bC{{\mathbf C}}
\newcommand\bD{{\mathbf D}}
\newcommand\bE{{\mathbf E}}
\newcommand\bF{{\mathbf F}}
\newcommand\bG{{\mathbf G}}
\newcommand\bH{{\mathbf H}}
\newcommand\bI{{\mathbf I}}
\newcommand\bJ{{\mathbf J}}
\newcommand\bK{{\mathbf K}}
\newcommand\bL{{\mathbf L}}
\newcommand\bM{{\mathbf M}}
\newcommand\bN{{\mathbf N}}
\newcommand\bO{{\mathbf O}}
\newcommand\bP{{\mathbf P}}
\newcommand\bQ{{\mathbf Q}}
\newcommand\bR{{\mathbf R}}
\newcommand\bS{{\mathbf S}}
\newcommand\bT{{\mathbf T}}
\newcommand\bU{{\mathbf U}}
\newcommand\bV{{\mathbf V}}
\newcommand\bW{{\mathbf W}}
\newcommand\bX{{\mathbf X}}
\newcommand\bY{{\mathbf Y}}
\newcommand\bZ{{\mathbf Z}}
\newcommand\bDelta{{\mathbf \Delta}}
\newcommand\bEta{{\mathbf \Eta}}
\newcommand\bKappa{{\mathbf \kappa}}%\Kappa does not exist...
\newcommand\bXi{{\mathbf \Xi}}
\newcommand\bOm{{\mathbf \Omega}}
\newcommand{\bmu}{\bm \mu}
\newcommand{\bnu}{\bm \nu}

%%%%%%%%%%%%

\newcommand\bfa{{\bm a}}
\newcommand\bfb{{\bm b}}
\newcommand\bfc{{\bm c}}
\newcommand\bfd{{\bm d}}
\newcommand\bfe{{\bm e}}
\newcommand\bff{{\bm f}}
\newcommand\bfg{{\bm g}}
\newcommand\bfh{{\bm h}}
\newcommand\bfi{{\bm i}}
\newcommand\bfj{{\bm j}}
\newcommand\bfk{{\bm k}}
\newcommand\bfl{{\bm l}}
\newcommand\bfm{{\bm m}}
\newcommand\bfn{{\bm n}}
\newcommand\bfo{{\bm o}}
\newcommand\bfp{{\bm p}}
\newcommand\bfq{{\bm q}}
\newcommand\bfr{{\bm r}}
\newcommand\bfs{{\bm s}}
\newcommand\bft{{\bm t}}
\newcommand\bfu{{\bm u}}
\newcommand\bfv{{\bm v}}
\newcommand\bfw{{\bm w}}
\newcommand\bfx{{\bm x}}
\newcommand\bfy{{\bm y}}
\newcommand\bfz{{\bm z}}
\newcommand\bfdelta{{\bm \delta}}
\newcommand\bfeta{{\bm \eta}}
\newcommand\bfkappa{{\bm \kappa}}
\newcommand\bftau{{\bm \tau}}
\newcommand\bfxi{{\bm \xi}}
\newcommand\bfom{{\bm \omega}}

%%%%%%%%%%%%

\newcommand\ubA{{\underline \bA}}
\newcommand\ubB{{\underline \bB}}
\newcommand\ubC{{\underline \bC}}
\newcommand\ubD{{\underline \bD}}
\newcommand\ubE{{\underline \bE}}
\newcommand\ubF{{\underline \bF}}
\newcommand\ubG{{\underline \bG}}
\newcommand\ubH{{\underline \bH}}
\newcommand\ubI{{\underline \bI}}
\newcommand\ubJ{{\underline \bJ}}
\newcommand\ubK{{\underline \bK}}
\newcommand\ubL{{\underline \bL}}
\newcommand\ubM{{\underline \bM}}
\newcommand\ubN{{\underline \bN}}
\newcommand\ubO{{\underline \bO}}
\newcommand\ubP{{\underline \bP}}
\newcommand\ubQ{{\underline \bQ}}
\newcommand\ubR{{\underline \bR}}
\newcommand\ubS{{\underline \bS}}
\newcommand\ubT{{\underline \bT}}
\newcommand\ubU{{\underline \bU}}
\newcommand\ubV{{\underline \bV}}
\newcommand\ubW{{\underline \bW}}
\newcommand\ubX{{\underline \bX}}
\newcommand\ubY{{\underline \bY}}
\newcommand\ubZ{{\underline \bZ}}
\newcommand\ubEta{{\underline \bEta}}
\newcommand\ubKappa{{\underline \bKappa}}
\newcommand\ubXi{{\underline \bXi}}
\newcommand\ubOm{{\underline \bOm}}

%%%%%%%%%%%%

\newcommand\uba{{\underline \bfa}}
\newcommand\ubb{{\underline \bfb}}
\newcommand\ubc{{\underline \bfc}}
\newcommand\ubd{{\underline \bfd}}
\newcommand\ube{{\underline \bfe}}
\newcommand\ubf{{\underline \bff}}
\newcommand\ubg{{\underline \bfg}}
\newcommand\ubh{{\underline \bfh}}
\newcommand\ubi{{\underline \bfi}}
\newcommand\ubj{{\underline \bfj}}
\newcommand\ubk{{\underline \bfk}}
\newcommand\ubl{{\underline \bfl}}
\newcommand\ubm{{\underline \bfm}}
\newcommand\ubn{{\underline \bfn}}
\newcommand\ubo{{\underline \bno}}
\newcommand\ubp{{\underline \bfp}}
\newcommand\ubq{{\underline \bfq}}
\newcommand\ubr{{\underline \bfr}}
\newcommand\ubs{{\underline \bfs}}
\newcommand\ubt{{\underline \bft}}
\newcommand\ubu{{\underline \bfu}}
\newcommand\ubv{{\underline \bfv}}
\newcommand\ubw{{\underline \bfw}}
\newcommand\ubx{{\underline \bfx}}
\newcommand\uby{{\underline \bfy}}
\newcommand\ubz{{\underline \bfz}}
\newcommand\ubeta{{\underline \bfeta}}
\newcommand\ubkappa{{\underline \bfkappa}}
\newcommand\ubxi{{\underline \bfxi}}
\newcommand\ubom{{\underline \bfom}}

%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\uA{{\underline A}}
\newcommand\uB{{\underline B}}
\newcommand\uC{{\underline C}}
\newcommand\uD{{\underline D}}
\newcommand\uE{{\underline E}}
\newcommand\uF{{\underline F}}
\newcommand\uG{{\underline G}}
\newcommand\uH{{\underline H}}
\newcommand\uI{{\underline I}}
\newcommand\uJ{{\underline J}}
\newcommand\uK{{\underline K}}
\newcommand\uL{{\underline L}}
\newcommand\uM{{\underline M}}
\newcommand\uN{{\underline N}}
\newcommand\uO{{\underline O}}
\newcommand\uP{{\underline P}}
\newcommand\uQ{{\underline Q}}
\newcommand\uR{{\underline R}}
\newcommand\uS{{\underline S}}
\newcommand\uT{{\underline T}}
\newcommand\uU{{\underline U}}
\newcommand\uV{{\underline V}}
\newcommand\uW{{\underline W}}
\newcommand\uX{{\underline X}}
\newcommand\uY{{\underline Y}}
\newcommand\uZ{{\underline Z}}
\newcommand\uGamma{{\underline \Gamma}}
\newcommand\uDelta{{\underline \Delta}}
\newcommand\uTheta{{\underline \Theta}}
\newcommand\uLambda{{\underline \Lambda}}
\newcommand\uXi{{\underline \Xi}}
\newcommand\uPi{{\underline \Pi}}
\newcommand\uSigma{{\underline \Sigma}}
\newcommand\uUpsilon{{\underline \Upsilon}}
\newcommand\uPhi{{\underline \Phi}}
\newcommand\uPsi{{\underline \Psi}}
\newcommand\uOm{{\underline \Omega}}

%%%%%%%%%%%%

\newcommand\ua{{\underline a}}
\newcommand\ub{{\underline b}}
\newcommand\uc{{\underline c}}
\newcommand\ud{{\underline d}}
\newcommand\ue{{\underline e}}
\newcommand\uf{{\underline f}}
\newcommand\ug{{\underline g}}
\newcommand\uh{{\underline h}}
\newcommand\ui{{\underline i}}
\newcommand\uj{{\underline j}}
\newcommand\uk{{\underline k}}
\newcommand\ul{{\underline l}}
\newcommand\um{{\underline m}}
\newcommand\un{{\underline n}}
\newcommand\uo{{\underline o}}
\newcommand\uup{{\underline p}}
\newcommand\uuq{{\underline q}}
\newcommand\ur{{\underline r}}
\newcommand\us{{\underline s}}
\newcommand\ut{{\underline t}}
\newcommand\uu{{\underline u}}
\newcommand\uv{{\underline v}}
\newcommand\uw{{\underline w}}
\newcommand\ux{{\underline x}}
\newcommand\uy{{\underline y}}
\newcommand\uz{{\underline z}}
\newcommand\ualpha{{\underline \alpha}}
\newcommand\uubeta{{\underline \beta}}
\newcommand\ugamma{{\underline \gamma}}
\newcommand\udelta{{\underline \delta}}
\newcommand\ueps{{\underline \epsilon}}
\newcommand\uvareps{{\underline \varepsilon}}
\newcommand\uzeta{{\underline \zeta}}
\newcommand\ueta{{\underline \eta}}
\newcommand\utheta{{\underline \theta}}
\newcommand\uvartheta{{\underline \vartheta}}
\newcommand\ukappa{{\underline \kappa}}
\newcommand\ulambda{{\underline \lambda}}
\newcommand\umu{{\underline \mu}}
\newcommand\unu{{\underline \nu}}
\newcommand\uxi{{\underline \xi}}
\newcommand\upi{{\underline \pi}}
\newcommand\uvarpi{{\underline \varpi}}
\newcommand\urho{{\underline \rho}}
\newcommand\uvarrho{{\underline \varrho}}
\newcommand\usigma{{\underline \sigma}}
\newcommand\uvarsigma{{\underline \varsigma}}
\newcommand\utau{{\underline \tau}}
\newcommand\uupsilon{{\underline \upsilon}}
\newcommand\uphi{{\underline \phi}}
\newcommand\uvarphi{{\underline \varphi}}
\newcommand\uchi{{\underline \chi}}
\newcommand\upsi{{\underline \psi}}
\newcommand\uom{{\underline \omega}}

%%%%%%%%%%%%

\newcommand\cA{{\mathcal A}}
\newcommand\cB{{\mathcal B}}
\newcommand\cC{{\mathcal C}}
\newcommand\cD{{\mathcal D}}
\newcommand\cE{{\mathcal E}}
\newcommand\cF{{\mathcal F}}
\newcommand\cG{{\mathcal G}}
\newcommand\cH{{\mathcal H}}
\newcommand\cI{{\mathcal I}}
\newcommand\cJ{{\mathcal J}}
\newcommand\cK{{\mathcal K}}
\newcommand\cL{{\mathcal L}}
\newcommand\cM{{\mathcal M}}
\newcommand\cN{{\mathcal N}}
\newcommand\cO{{\mathcal O}}
\newcommand\cP{{\mathcal P}}
\newcommand\cQ{{\mathcal Q}}
\newcommand\cR{{\mathcal R}}
\newcommand\cS{{\mathcal S}}
\newcommand\cT{{\mathcal T}}
\newcommand\cU{{\mathcal U}}
\newcommand\cV{{\mathcal V}}
\newcommand\cW{{\mathcal W}}
\newcommand\cX{{\mathcal X}}
\newcommand\cY{{\mathcal Y}}
\newcommand\cZ{{\mathcal Z}}
\newcommand\scP{{\mathscr P}}
\newcommand\scC{{\mathscr C}}
%%%%%%%%%%%%

\newcommand\ta{{\widetilde a}}
\newcommand\tb{{\widetilde b}}
\newcommand\tc{{\widetilde c}}
\newcommand\td{{\widetilde d}}
\newcommand\te{{\widetilde e}}
\newcommand\tf{{\widetilde f}}
\newcommand\tg{{\widetilde g}}
\newcommand\tth{{\widetilde h}}
\newcommand\ti{{\widetilde i}}
\newcommand\tj{{\widetilde j}}
\newcommand\tk{{\widetilde k}}
\newcommand\tl{{\widetilde l}}
\newcommand\tm{{\widetilde m}}
\newcommand\tn{{\widetilde n}}
\newcommand\tto{{\widetilde o}}
\newcommand\tp{{\widetilde p}}
\newcommand\tq{{\widetilde q}}
\newcommand\tr{{\widetilde r}}
\newcommand\ts{{\widetilde s}}
\newcommand\ttt{{\widetilde t}}
\newcommand\tu{{\widetilde u}}
\newcommand\tv{{\widetilde v}}
\newcommand\tw{{\widetilde w}}
\newcommand\tx{{\widetilde x}}
\newcommand\ty{{\widetilde y}}
\newcommand\tz{{\widetilde z}}
\newcommand\talpha{{\widetilde \alpha}}
\newcommand\tbeta{{\widetilde \beta}}
\newcommand\tgamma{{\widetilde \gamma}}
\newcommand\tdelta{{\widetilde \delta}}
\newcommand\teps{{\widetilde \epsilon}}
\newcommand\tvareps{{\widetilde \varepsilon}}
\newcommand\tzeta{{\widetilde \zeta}}
\newcommand\teta{{\widetilde \eta}}
\newcommand\ttheta{{\widetilde \theta}}
\newcommand\tvartheta{{\widetilde \vartheta}}
\newcommand\tkappa{{\widetilde \kappa}}
\newcommand\tlambda{{\widetilde \lambda}}
\newcommand\tmu{{\widetilde \mu}}
\newcommand\tnu{{\widetilde \nu}}
\newcommand\txi{{\widetilde \xi}}
\newcommand\tpi{{\widetilde \pi}}
\newcommand\tvarpi{{\widetilde \varpi}}
\newcommand\trho{{\widetilde \rho}}
\newcommand\tvarrho{{\widetilde \varrho}}
\newcommand\tsigma{{\widetilde \sigma}}
\newcommand\tvarsigma{{\widetilde \varsigma}}
\newcommand\ttau{{\widetilde \tau}}
\newcommand\tupsilon{{\widetilde \upsilon}}
\newcommand\tphi{{\widetilde \phi}}
\newcommand\tvarphi{{\widetilde \varphi}}
\newcommand\tchi{{\widetilde \chi}}
\newcommand\tpsi{{\widetilde \psi}}
\newcommand\tom{{\widetilde \omega}}

%%%%%%%%%%%%

\newcommand\tA{\widetilde{A}}
\newcommand\tB{\widetilde{B}}
\newcommand\tC{\widetilde{C}}
\newcommand\tD{\widetilde{D}}
\newcommand\tE{\widetilde{E}}
\newcommand\tG{\widetilde{G}}
\newcommand\tH{\widetilde{H}}
\newcommand\tI{\widetilde{I}}
\newcommand\tJ{\widetilde{J}}
\newcommand\tK{\widetilde{K}}
\newcommand\tL{\widetilde{L}}
\newcommand\tM{\widetilde{M}}
\newcommand\tN{\widetilde{N}}
\newcommand\tO{\widetilde{O}}
\newcommand\tP{\widetilde{P}}
\newcommand\tQ{\widetilde{Q}}
\newcommand\tR{\widetilde{R}}
\newcommand\tS{\widetilde{S}}
\newcommand\tT{\widetilde{T}}
\newcommand\tU{\widetilde{U}}
\newcommand\tV{\widetilde{V}}
\newcommand\tW{\widetilde{W}}
\newcommand\tX{\widetilde{X}}
\newcommand\tY{\widetilde{Y}}
\newcommand\tZ{\widetilde{Z}}
\newcommand\tGamma{\widetilde{\Gamma}}
\newcommand\tDelta{\widetilde{\Delta}}
\newcommand\tTheta{\widetilde{\Theta}}
\newcommand\tLambda{\widetilde{\Lambda}}
\newcommand\tXi{\widetilde{\Xi}}
\newcommand\tPi{\widetilde{\Pi}}
\newcommand\tSigma{\widetilde{\Sigma}}
\newcommand\tUpsilon{\widetilde{\Upsilon}}
\newcommand\tPhi{\widetilde{\Phi}}
\newcommand\tPsi{\widetilde{\Psi}}
\newcommand\tOm{\widetilde{\Omega}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\tba{\widetilde{\bfa}}
\newcommand\tbb{\widetilde{\bfb}}
\newcommand\tbc{\widetilde{\bfc}}
\newcommand\tbd{\widetilde{\bfd}}
\newcommand\tbe{\widetilde{\bfe}}
\newcommand\tbf{\widetilde{\bff}}
\newcommand\tbg{\widetilde{\bfg}}
\newcommand\tbh{\widetilde{\bfh}}
\newcommand\tbi{\widetilde{\bfi}}
\newcommand\tbj{\widetilde{\bfj}}
\newcommand\tbk{\widetilde{\bfk}}
\newcommand\tbl{\widetilde{\bfl}}
\newcommand\tbm{\widetilde{\bfm}}
\newcommand\tbn{\widetilde{\bfn}}
\newcommand\tbo{\widetilde{\bno}}
\newcommand\tbp{\widetilde{\bfp}}
\newcommand\tbq{\widetilde{\bfq}}
\newcommand\tbr{\widetilde{\bfr}}
\newcommand\tbs{\widetilde{\bfs}}
\newcommand\tbt{\widetilde{\bft}}
\newcommand\tbu{\widetilde{\bfu}}
\newcommand\tbv{\widetilde{\bfv}}
\newcommand\tbw{\widetilde{\bfw}}
\newcommand\tbx{\widetilde{\bfx}}
\newcommand\tby{\widetilde{\bfy}}
\newcommand\tbz{\widetilde{\bfz}}
\newcommand\tbalpha{\widetilde{\bfalpha}}
\newcommand\tbbeta{\widetilde{\bfbeta}}
\newcommand\tbgamma{\widetilde{\bfgamma}}
\newcommand\tbdelta{\widetilde{\bfdelta}}
\newcommand\tbeps{\widetilde{\bfeps}}
\newcommand\tbvareps{\widetilde{\bfvareps}}
\newcommand\tbzeta{\widetilde{\bfzeta}}
\newcommand\tbtbeta{\widetilde{\bfeta}}
\newcommand\tbtheta{\widetilde{\bftheta}}
\newcommand\tbvartheta{\widetilde{\bfvartheta}}
\newcommand\tbkappa{\widetilde{\bfkappa}}
\newcommand\tblambda{\widetilde{\bflambda}}
\newcommand\tbmu{\widetilde{\bfmu}}
\newcommand\tbnu{\widetilde{\bfnu}}
\newcommand\tbxi{\widetilde{\bfxi}}
\newcommand\tbpi{\widetilde{\bfpi}}
\newcommand\tbvarpi{\widetilde{\bfvarpi}}
\newcommand\tbrho{\widetilde{\bfrho}}
\newcommand\tbvarrho{\widetilde{\bfvarrho}}
\newcommand\tbsigma{\widetilde{\bfsigma}}
\newcommand\tbvarsigma{\widetilde{\bfvarsigma}}
\newcommand\tbtau{\widetilde{\bftau}}
\newcommand\tbupsilon{\widetilde{\bfupsilon}}
\newcommand\tbphi{\widetilde{\bfphi}}
\newcommand\tbvarphi{\widetilde{\bfvarphi}}
\newcommand\tbchi{\widetilde{\bfchi}}
\newcommand\tbpsi{\widetilde{\bfpsi}}
\newcommand\tbom{\widetilde{\bfom}}

%%%%%%%%%%%%

\newcommand\tbA{\widetilde{\bA}}
\newcommand\tbB{\widetilde{\bB}}
\newcommand\tbC{\widetilde{\bC}}
\newcommand\tbD{\widetilde{\bD}}
\newcommand\tbE{\widetilde{\bE}}
\newcommand\tbF{\widetilde{\bF}}
\newcommand\tbG{\widetilde{\bG}}
\newcommand\tbH{\widetilde{\bH}}
\newcommand\tbI{\widetilde{\bI}}
\newcommand\tbJ{\widetilde{\bJ}}
\newcommand\tbK{\widetilde{\bK}}
\newcommand\tbL{\widetilde{\bL}}
\newcommand\tbM{\widetilde{\bM}}
\newcommand\tbN{\widetilde{\bN}}
\newcommand\tbO{\widetilde{\bO}}
\newcommand\tbP{\widetilde{\bP}}
\newcommand\tbQ{\widetilde{\bQ}}
\newcommand\tbR{\widetilde{\bR}}
\newcommand\tbS{\widetilde{\bS}}
\newcommand\tbT{\widetilde{\bT}}
\newcommand\tbU{\widetilde{\bU}}
\newcommand\tbV{\widetilde{\bV}}
\newcommand\tbW{\widetilde{\bW}}
\newcommand\tbX{\widetilde{\bX}}
\newcommand\tbY{\widetilde{\bY}}
\newcommand\tbZ{\widetilde{\bZ}}
\newcommand\tbGamma{\widetilde{\bGamma}}
\newcommand\tbDelta{\widetilde{\bDelta}}
\newcommand\tbTheta{\widetilde{\bTheta}}
\newcommand\tbLambda{\widetilde{\bLambda}}
\newcommand\tbXi{\widetilde{\bXi}}
\newcommand\tbPi{\widetilde{\bPi}}
\newcommand\tbSigma{\widetilde{\bSigma}}
\newcommand\tbUpsilon{\widetilde{\bUpsilon}}
\newcommand\tbPhi{\widetilde{\bPhi}}
\newcommand\tbPsi{\widetilde{\bPsi}}
\newcommand\tbOm{\widetilde{\bOm}}


%%%%%%%%%%%%%%%
\newcommand\eDr{\eD_{\textrm{r}}}
\newcommand\eDt{\eD_{\textrm{\theta}}}

%%%%%%%%%%%%%%%
\newcommand{\ttime}{\widetilde{t}}
\newcommand{\ttauv}{\widetilde{\bftau}_{\bv}}
\newcommand{\htime}{\widehat{t}}
\newcommand{\hx}{\widehat{\bfx}}
\newcommand{\hy}{\widehat{\bfy}}
\newcommand{\hv}{\widehat{\bfv}}
\newcommand{\hw}{\widehat{\bfw}}
\newcommand{\htauy}{\widehat{\bftau}_{\bfy}}
\newcommand{\htauv}{\widehat{\bftau}_{\bfv}}

%%%%%%%%%%%%%%%
\newcommand{\Dt}{\Delta t}

\newcommand{\llangle}{\left\langle}
\newcommand{\rrangle}{\right\rangle}
\newcommand\Supp{\textrm{Supp}}
\newcommand{\poly}{\cH}
\newcommand{\proj}{\cI}


